Weak amenability for Fourier algebras of 1-connected nilpotent Lie groups

A special case of a conjecture raised by Forrest and Runde (Math. Zeit., 2005) asserts that the Fourier algebra of every non-abelian connected Lie group fails to be weakly amenable; this was aleady known to hold in the non-abelian compact cases, by earlier work of Johnson (JLMS, 1994) and Plymen (unpublished note). In recent work (JFA, 2014) the present authors verified this conjecture for the real ax+b group and hence, by structure theory, for any semisimple Lie group. In this paper we verify the conjecture for all 1-connected, non-abelian nilpotent Lie groups, by reducing the problem to the case of the Heisenberg group. As in our previous paper, an explicit non-zero derivation is constructed on a dense subalgebra, and then shown to be bounded using harmonic analysis. En route, we use the known fusion rules for Schr\"odinger representations to give a concrete realization of the "dual convolution" for this group as a kind of twisted, operator-valued convolution. We also give some partial results for solvable groups which give further evidence to support the general conjecture.

==> WAAHmac2.tex <==
\NeedsTeXFormat{LaTeX2e}
\RequirePackage{amsmath,amssymb,amsfonts}
\numberwithin{equation}{section}


%------------


\RequirePackage{amsthm}   %Inbuilt environments for defns etc
%\usepackage{theorem}

\newcounter{pulse}[section]
\numberwithin{pulse}{section}  % all thms, etc set from pulse


%Styles for theorems, definitions, remarks

\newcommand{\thf}{\sc} % alias for theorem heading font

%-Theorems
\theoremstyle{plain}
\newtheorem{thm}[pulse]{\thf Theorem}
\newtheorem*{thmstar}{\thf Theorem}
\newtheorem{prop}[pulse]{\thf Proposition}
\newtheorem{lem}[pulse]{\thf Lemma}
\newtheorem{cor}[pulse]{\thf Corollary}
%-Definitions
\theoremstyle{definition}
\newtheorem{dfn}[pulse]{\thf Definition}
\newtheorem*{notn}{\thf Notation}
\newtheorem{eg}[pulse]{\thf Example}
%-Remarks
\theoremstyle{remark}
\newtheorem{rem}[pulse]{\thf Remark}
\newtheorem*{remstar}{\thf Remark}


\renewcommand{\emph}[1]{{\sl #1}\/} % use slanted font for emphasis
%\newcommand{\st}{\;:\;}
\newcommand{\defeq}{:=}
\newcommand{\sid}{\operatorname{\sf id}}  % generic notation for identity map


% Fourier algebra, etc
\newcommand{\FA}{\operatorname{A}}
\newcommand{\FS}{\operatorname{B}}
\newcommand{\VN}{\operatorname{VN}}
\newcommand{\Cst}{\operatorname{C}^*}

% Various generic letters in different fonts
%% calligraphic
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
% ordinary bold
%\newcommand{\bF}{{\bf F}}
%\newcommand{\bV}{{\bf V}}
\newcommand{\bx}{{\bf x}}
%% sans-serif
\newcommand{\sB}{{\sf B}}
\newcommand{\sH}{{\sf H}}
\newcommand{\sK}{{\sf K}}
\newcommand{\sM}{{\sf M}}
\newcommand{\sW}{{\sf W}}
%% blackboard bold
\newcommand{\bbI}{{\mathbb I}}
\newcommand{\bbJ}{{\mathbb J}}

% Special objects (in the Bourbaki sense)
\newcommand{\Cplx}{\mathbb C}
\newcommand{\bbH}{{\mathbb H}} % Heisenberg group (unpolarized)
\newcommand{\Hpol}{\bbH_{\rm pol}} % polarized Heisenberg group
\newcommand{\Nat}{\mathbb N}
\newcommand{\Rat}{\mathbb Q}
\newcommand{\Real}{\mathbb R}
\newcommand{\Torus}{\mathbb T} %Unit circle
\newcommand{\Zahl}{\mathbb Z}

%% abbreviations for Greek letters
\newcommand{\lm}{\lambda}


%--------------------------------------------


% journals seem to want upright roman numerals in numbered lists, we need to force this if in an italic environment
\newenvironment{newnum}{%
\begin{enumerate}
\renewcommand{\labelenumi}{{\rm(\roman{enumi})}}
\renewcommand{\theenumi}{{\rm(\roman{enumi})}}
}{\end{enumerate}\ignorespacesafterend}

\newcommand{\twomat}[4]{{\begin{pmatrix} #1 & #2 \\ #3 & #4     \end{pmatrix}}}
   
%%Personal preference and fundamentals
\newcommand{\veps}{\varepsilon}
\newcommand{\wtild}{\widetilde}
\newcommand{\what}{\widehat}
\newcommand{\blob}{\bullet}
\newcommand{\blank}{\underline{\quad}}
\newcommand{\iso}{\cong}
\renewcommand{\Re}{\operatorname{\sf Re}}
\renewcommand{\Im}{\operatorname{\sf Im}}
%\DeclareMathOperator{\op}{op}
\newcommand{\id}[1][]{{\sf 1}_{#1}} % identity of group, algebra, object in category
\newcommand{\wstar}{\ensuremath{{\rm w}^*}}

\newcommand{\tr}{\operatorname{Tr}} % matrix trace
\newcommand{\Tr}{\operatorname{Tr}} % matrix trace
\newcommand{\spec}{\operatorname{sp}} % spectrum
\newcommand{\pair}[2]{\langle{#1},\,{#2}\rangle}
\newcommand{\supp}{\operatorname{supp}}

\newcommand{\abs}[1]{\vert{#1}\vert}
\newcommand{\norm}[1]{\Vert{#1}\Vert}

\newcommand{\lin}{\operatorname{lin}}
\newcommand{\ip}[2]{\langle{#1},\,{#2}\rangle}


% Tensor products etc.
\newcommand{\tp}{\mathbin{\otimes}}
\newcommand{\ptp}{\mathbin{\widehat{\otimes}}} % projective tensor product
\newcommand{\optp}{\mathbin{\widehat{\otimes}}_{\rm op}} % OS projective tensor product


% Misc
\newcommand{\clin}{\overline{\rm lin}} %closed linear span
\newcommand{\Ind}{{\rm Ind}} %induced representation
\newcommand{\ind}{\operatorname{Ind}}
\newcommand{\Bdd}{{\mathcal B}}

%% Various Lie groups (group schemes?)
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\OO}{\operatorname{O}}
\newcommand{\Euc}{\operatorname{Euc}}
%\newcommand{\SOTHREE}{\SO(3)} % idea is that we can always change our convention/abbreviation if we need to
%\newcommand{\SUTWO}{\SU(2)} % idea is that we can always change our convention/abbreviation if we need to


% ad hoc
\newcommand{\Trig}{\operatorname{Trig}}
\newcommand{\eith}{e^{i\theta}}
\newcommand{\sch}{{\sf Sch}} % Schr\"odinger reps
\newcommand{\dd}{\partial}
\newcommand{\dbydz}[1]{\frac{\partial#1}{\partial z}}
%\newcommand{\dhat}{\widehat{\partial}}
\newcommand{\STN}{{\sf S}} % Schatten class operators
\newcommand{\conull}{{\mathcal O}} % conull set of the unitary dual
\newcommand{\esssup}{\operatorname{ess.sup}}
\newcommand{\twoc}[2]{\left( \begin{matrix}#1\\ #2 \end{matrix}\right)}
\newcommand{\RR}{{\Real\times\Real}}
\newcommand{\st}{\mathbin{\colon}}


% stuff for Lie algebras and Lie groups
\newcommand{\lie}[1]{{\sf #1}}
\newcommand{\fa}{\lie{a}}
\newcommand{\fg}{\lie{g}}
\newcommand{\fh}{\lie{h}}
\newcommand{\fk}{\lie{k}}
\newcommand{\fn}{\lie{n}}
\newcommand{\fp}{\lie{p}}
\newcommand{\fr}{\lie{r}}
\newcommand{\fs}{\lie{s}}
\newcommand{\fsl}{\lie{sl}}
%\newcommand{\ad}{\operatorname{ad}}
%\newcommand{\Ad}{\operatorname{Ad}}
%\newcommand{\rad}{\operatorname{rad}}
%\newcommand{\Aff}{\operatorname{Aff}}



% just for making revisions
%\newcommand{\MGrem}[1]{\fbox{\textbf{[MG] \sf#1}}\marginpar{\sf FIX ME}}
%\newcommand{\YCrem}[1]{\fbox{\textbf{[YC] \sf#1}}\marginpar{\sf FIX ME}}


\newcommand{\opconv}{\mathbin{\sharp}}

\newcommand{\opnorm}[1]{\norm{#1}_\infty}
\newcommand{\wnorm}[1]{\norm{#1}_{\sf W}}
\newcommand{\mnorm}[1]{\norm{#1}_{\sf M}}

% ---------------------------------------

% function spaces associated to Heisenberg group

\newcommand{\hrdual}{\widehat{\bbH}_r}  % OLD COMMAND KEPT FOR LEGACY
%\newcommand{\Hdual}[1]{L^{#1}(\hrdual, \STN_{#1})}
\newcommand{\FAH}{\FA(\bbH)}
\newcommand{\LRS}{L^1(\Real,\STN_1)}
\newcommand{\LIRS}{L^\infty(\Real,\STN_1)}
\newcommand{\LRB}{L^1(\Real,\sB)}
\newcommand{\LRK}{L^1(\Real,\sK)}
\newcommand{\CCRS}{C_c(\Real,\STN_1)}

